An Algebraic Framework for the Real-Time Solution of Inverse Problems on Embedded Systems

This article presents a new approach to the real-time solution of inverse problems on embedded systems. The class of problems addressed corresponds to ordinary differential equations (ODEs) with generalized linear constraints, whereby the data from an array of sensors forms the forcing function. The solution of the equation is formulated as a least squares (LS) problem with linear constraints. The LS approach makes the method suitable for the explicit solution of inverse problems where the forcing function is perturbed by noise. The algebraic computation is partitioned into a initial preparatory step, which precomputes the matrices required for the run-time computation; and the cyclic run-time computation, which is repeated with each acquisition of sensor data. The cyclic computation consists of a single matrix-vector multiplication, in this manner computation complexity is known a-priori, fulfilling the definition of a real-time computation. Numerical testing of the new method is presented on perturbed as well as unperturbed problems; the results are compared with known analytic solutions and solutions acquired from state-of-the-art implicit solvers. The solution is implemented with model based design and uses only fundamental linear algebra; consequently, this approach supports automatic code generation for deployment on embedded systems. The targeting concept was tested via software- and processor-in-the-loop verification on two systems with different processor architectures. Finally, the method was tested on a laboratory prototype with real measurement data for the monitoring of flexible structures. The problem solved is: the real-time overconstrained reconstruction of a curve from measured gradients. Such systems are commonly encountered in the monitoring of structures and/or ground subsidence.

==> setListings.tex <==
% setup the listings package
\lstset{language=Matlab,basicstyle=\small\ttfamily,
commentstyle=\color[rgb]{.133,.545,.133}\small\ttfamily,
keywordstyle=\color[rgb]{0,0,1}\ttfamily\small,
stringstyle=\color[rgb]{.627,.126,.941}\ttfamily\small,
showstringspaces=false,
xleftmargin=0.8cm,resetmargins=true,escapechar=\$,captionpos=b,
breaklines=true,breakatwhitespace=false,breakindent=2cm
,numbers=left,numbersep=2ex,numberstyle=\small\ttfamily,
columns=flexible,literate=
    *{=}{{$ = $}}1
    %{'}{{$^T$}}1
    {&}{AND}3
    {|}{OR}2
    {||}{OR}2
    {&&}{AND}3
    {~}{NOT}3
    {==}{$=$}1
    {<=}{{$\leq$}}1
    {>=}{{$\geq$}}1
    {~=}{{$\neq$}}1
}
